Graded transcendental functions: an application to four-point amplitudes with one off-shell leg

Several recent works have demonstrated the powerful algebraic simplifications that can be achieved for scattering amplitudes through a systematic grading of transcendental quantities. We develop these concepts to construct a minimal basis of functions tailored to a scattering amplitude in a general way. Starting with formal solutions for all master integral topologies, we organise the appearing functions by properties such as their symbol alphabet or letter adjacency. We rotate the basis such that functions with spurious features appear in the least possible number of basis elements. Since their coefficients must vanish for physical quantities, this approach avoids complex cancellations. As a first application, we evaluate all integral topologies relevant to the three-loop $Hggg$ and $Hgq\bar{q}$ amplitudes in the leading-colour approximation and heavy-top limit. We describe the derivation of canonical differential equation systems and present a method for fixing boundary conditions without the need for a full functional representation. Using multiple numerical reductions, we test the maximal transcendentality conjecture for $Hggg$ and identify a new letter which appears in functions of weight 4 and 5. In addition, we provide the first direct analytic computation of a three-point form factor of the operator $\mathrm{Tr}(\phi^2)$ in planar $\mathcal{N}=4$ sYM and find agreement with numerical and bootstrapped results.

==> Figures/triangle.tex <==
\begin{figure}[h]
\noindent\begin{minipage}{\linewidth}
\centering
\includegraphics[width=0.7\textwidth]{Imports/paths_v2.pdf}
\renewcommand{\arraystretch}{1.05}
\centering
\begin{tabular}{llll}
\multicolumn{1}{l}{segment} & start-/end-point & \multicolumn{1}{l}{$x(t,\delta)$ } & \multicolumn{1}{l}{$y(t,\delta)$ }\\ \hline
\multicolumn{1}{l}{ $\quad$  I} & $P_1 \rightarrow P_2$& \multicolumn{1}{l}{$t$} & \multicolumn{1}{l}{$\delta$}   \\ \hline
\multicolumn{1}{l}{ $\quad$  II} & $P_2 \rightarrow P_3$ & \multicolumn{1}{l}{$1-\delta \left[(1-t)^2 + t^2\right]$} & \multicolumn{1}{l}{$\delta t^2$}  \\ \hline
\multicolumn{1}{l}{ $\quad$  III} & $P_3 \rightarrow P_4$& \multicolumn{1}{l}{$1-t-\delta$} & \multicolumn{1}{l}{$t$} \\ \hline
\multicolumn{1}{l}{ $\quad$  IV} & $P_4 \rightarrow P_5$& \multicolumn{1}{l}{$\delta (1-t)^2$} & \multicolumn{1}{l}{$1-\delta \left[(1-t)^2 + t^2)\right]$}  \\ \hline
\multicolumn{1}{l}{ $\quad$  V} & $P_5 \rightarrow P_6$& \multicolumn{1}{l}{$\delta$} & \multicolumn{1}{l}{$1-t$}  \\ \hline
\multicolumn{1}{l}{ $\quad$  VI}& $P_6 \rightarrow P_1$ & \multicolumn{1}{l}{$\delta t^2$} & \multicolumn{1}{l}{$\delta (1-t)^2$}  \\ \hline
\end{tabular}
\captionof{figure}{Single-variable kinematic slices used in the determination of boundary constants. 
The Euclidean region is the triangle enclosed by black lines. 
Segments I,II,III IV,V,VI (red) are infinitesimally close to the branch lines. 
The blue arrows indicate analytic continuation outside the Euclidean region in order to connect the red and blue segments. 
Blue segments correspond to regular slices, where an infinitesimal displacement is not needed. 
The table summarizes the parametrization of each segment in terms of the two new parameters with values  $\delta\rightarrow 0^+$ and $  t\in(0,1)$. 
Start-/end-points $P_1, \dots, P_6$ in the circles. 
Point $P_7, P_8, P_9$ allows for matching between the inner triangle and the regular limit $x=-y, y=1, x=1$.}
\label{fig:segments boundary}
\end{minipage}
\end{figure}
